On the Number of Maximal Cliques in Two-Dimensional Random Geometric Graphs: Euclidean and Hyperbolic

Maximal clique enumeration appears in various real-world networks, such as social networks and protein-protein interaction networks for different applications. For general graph inputs, the number of maximal cliques can be up to $3^{|V|/3}$. However, many previous works suggest that the number is much smaller than that on real-world networks, and polynomial-delay algorithms enable us to enumerate them in a realistic-time span. To bridge the gap between the worst case and practice, we consider the number of maximal cliques in two popular models of real-world networks: Euclidean random geometric graphs and hyperbolic random graphs. We show that the number of maximal cliques on Euclidean random geometric graphs is lower and upper bounded by $\exp(\Omega(|V|^{1/3}))$ and $\exp(O(|V|^{1/3+\epsilon}))$ with high probability for any $\epsilon > 0$. For a hyperbolic random graph, we give the bounds of $\exp(\Omega(|V|^{(3-\gamma)/6}))$ and $\exp(O(|V|^{(3-\gamma+\epsilon)/6)}))$ where $\gamma$ is the power-law degree exponent between 2 and 3.

==> sections/sandbox.tex <==
\begin{comment}
Here I'll present my main result. I can give references \cite{ref2}, and 
I can write everything I want. I can even use figures but I remember 
that I have to send the .eps version of my figure 
(i.e. the file myfigure.eps) by e-mail to the organizers. 
\end{comment}


\begin{comment}
It can capture the structure of the whole graph.
Maximal clique enumeration [Akkoyunlu 1973; Bron and Kerbosch 1973] is a longstanding problem in graph theory. It is closely related to a number of fundamental graph
problems, such as maximal independent sets (or minimal vertex covers) [Tsukiyama
et al. 1977], graph coloring [Byskov 2003], maximal common induced subgraphs
[Koch 2001], maximal common edge subgraphs [Koch 2001], etc. Its significance is
not just limited to graph theory but also in numerous applications in various realworld networks, such as social network analysis [Faust and Wasserman 1995], hierarchy detection through email networks [Creamer et al. 2007], study of structures instances 
behavioral and cognitive networks [Bernard et al. 1979], statistical analysis of financial
networks [Boginski et al. 2005], clustering in dynamic networks [Stix 2004], the detection of emergent patterns in terrorist networks [Berry et al. 2004], as well as various
applications in computational biology [Abu-Khzam et al. 2005], including the detection of protein-protein interaction complex [Zhang et al. 2008] and clustering protein
sequences [Mohseni-Zadeh et al. 2004].
\par
Pattern counting is an important graph analysis tool in
many domains: anomaly detection, social network analysis,
bioinformatics among others [21, 27, 10, 29, 22, 17]. Many
real world graphs show significantly higher counts of certain
patterns than one would expect in a random graph [21, 46,
27]. This technique has been referred to with a variety of
names: subgraph analysis, motif counting, graphlet analysis,
etc. But the fundamental task is to count the occurrence
of a small pattern graph in a large input graph. In all
such applications, it is essential to have fast algorithms for
pattern counting.
It is well-known that certain patterns capture specific
semantic relationships, and thus the social dynamics are
reflected in these graph structures. The most famous such
pattern is the triangle, which consists of three vertices
connected to each other. Triangle counting has a rich history
in the social sciences and network science [21, 46, 10, 47].
We focus on the more general problem of clique counting.
A k-clique is a set of k vertices that are all connected to each
other; thus, a triangle is a 3-clique. Cliques are extremely
significant in social network analysis (Chap. 11 of [20] and
Chap. 2 of [23]). They are the archetypal example of a dense
subgraph, and a number of recent results use cliques to find
large, dense subregions of a network [32, 41, 28, 43].
\end{comment}

\begin{comment}
A Graph is an Abstraction of networks from different fields: social networks, web graphs,
protein-protein interaction networks.
Different tasks from different networks can be generalized to a common problem on graphs.
Especially, some tasks can often be described in terms of cliques and this is why the problems
are gathering attention. \par
A complete subgraph, clique corresponds to an important 
It is also used in general dense subgraph problems.
The cliques are used to find not only a complete subgraph also more general dense subgraphs.
$k$-clique densest subgraph discovery and nucleus decomposition.
$k$-clique densest subgraph discovery. This is the generalization of densest subgraph discovery.
nucleus decomposition. This is the generalization of core decomposition.
Counting triangles is a common problem, but also counting larger cliques are necessary to 
apply those methods. \par
Maximal clique enumeration is the task of listing cliques
appears in various kinds of real-world networks such as social
networks, web graphs, and protein-protein interaction networks for different applications. 
Not only does it have direct applications but also,
the algorithms and techniques of the problem are used for other clique tasks such as maximum clique problem,
clique percolations, and $k$-clique counting problem. \par
\end{comment}
\begin{comment}
The number of maximal cliques can be exponential to the number of vertices $n$ since Tur\`{a}n graph $T(n, r)$ has $(n/r)^r$ maximal cliques.
Especially, when $r=\lceil n/3 \rceil$, the number is maximum, and the graph is called the Moon-Moser graph.
Therefore, the enumeration can also take exponential time.
On the other hand, in real instances, the number is often much smaller than that.
of maximal cliques can be exponential to the number of vertices.
time even on a network with a few million vertices.
Combination of the classic maximal clique enumeration algorithm,
Bron-Kerbosch algorithm \cite{bron-kerbosch}, and graph orientation \cite{orientation} works very efficiently
even on networks with millions of vertices.
Also, there are algorithms called polynomial time delay algorithms whose running time is bounded as $O(poly(n) \mathcal{M}(G))$,
where $\mathcal{M}(G)$ is the number of maximal cliques in a graph $G$.
Those algorithms also works very fast practically. \par
There are works that try to account for this phenomenon. Degeneracy $d$ is a graph parameter
that is closely related to the graph orientation and dense subgraphs. Using the parameter, $\mathcal{M}(G)$ is bounded By
$O(n3^{d/3})$. Since the parameter is often around 50-500 even for networks with millions of vertices,
the bound works well. Also, we have $c$-closed graph \cite{closedness}. This parameter is inspired by 
the property of real-world networks called the triadic closure property:
if two vertices have many common neighbors, they are likely to be connected. 
It gives a bound of $O(n^2 3^{c/3})$ on $\mathcal{M}(G)$. Although
$c$ is completely different notation from $d$, experiments show that 
it is small on some networks, thus giving a modest bound on $\mathcal{M}(G)$. \par
Although their theoretical hardness, there are many works which are able to solve 
those clique problems on real-world networks, even for instances with millions of vertices. 
\end{comment}
\begin{comment}
In terms of clique number and the number of $k$-cliques, efforts are put into random graphs.
Euclidean random geometric graphs are thought to be good representations of protein-protein
interaction networks, since they have a high clustering coefficient (a measurement for triadic closure property).
The size of the maximum cliques and the number of $k$-cliques are studied.
Hyperbolic random graphs \cite{hyperbolic} are similar to Euclidean random geometric graphs except they are considered
on a plane with negative curvature. It seems like an odd idea to adopt a hyperbolic plane, but
this yields power-law degree distribution and a high clustering coefficient which are the
two most important properties of real-world networks. Thanks to its simple generation, many parameters are studied:
clique number, the number of $k$-cliques, diameter, treewidth, modularity, and so on.
To some extent, those theoretical results match the parameter values of real instances. \par
\end{comment}
\begin{comment}
The real-world networks are not completely random. They share some common properties.
First, they have power-law degree distribution:
the number of nodes with vertex degree $k$ is propotional to $k^{-\gamma}$. In many instances, $\gamma$ is between
two and three, and the graphs are called scale-free in this case. Second one is triadic closure property 
or high clustering coefficient.
if two vertices have common neighbor, then they are likely to be connected. The other properties are 
tree-like structure, small degeneracy, small diameter, small clique number and so on. \par

One model of real-world networks that has been proposed is the hyperbolic random graph. 
These graphs are generated by independently placing vertices according to a particular 
distribution in a two-dimensional space with negative curvature 
and connecting two vertices that are within a certain distance. 
Despite its simple generation process, it has common properties of real-world networks 
with high probability, such as a power-law degree distribution, high clustering coefficient, 
and small diameter. Furthermore, compared to other models of real-world networks, 
it is known that these graphs correctly predict the size of the maximum clique even in a sparse regime. \par
\end{comment}

